The Symmetry Coefficient of Positively Homogeneous Functions

The Bregman distance is a central tool in convex optimization, particularly in first-order gradient descent and proximal-based algorithms. Such methods enable optimization of functions without Lipschitz continuous gradients by leveraging the concept of relative smoothness, with respect to a reference function $h$. A key factor in determining the full range of allowed step sizes in Bregman schemes is the symmetry coefficient, $\alpha(h)$, of the reference function $h$. While some explicit values of $\alpha(h)$ have been determined for specific functions $h$, a general characterization has remained elusive. This paper explores two problems: ($\textit{i}$) deriving calculus rules for the symmetry coefficient and ($\textit{ii}$) computing $\alpha(\lVert\cdot\rVert_2^p)$ for general $p$. We establish upper and lower bounds for the symmetry coefficient of sums of positively homogeneous Legendre functions and, under certain conditions, provide exact formulas for these sums. Furthermore, we demonstrate that $\alpha(\lVert\cdot\rVert_2^p)$ is independent of dimension and propose an efficient algorithm for its computation. Additionally, we prove that $\alpha(\lVert\cdot\rVert_2^p)$ asymptotically equals, and is lower bounded by, the function $1/(2p)$, offering a simpler upper bound for step sizes in Bregman schemes. Finally, we present closed-form computations for specific cases such as $p \in \{6,8,10\}$.

==> data/data.tex <==
p,alpha
2.0,1.0
5.337792642140468,0.17265913955761725
8.675585284280936,0.08817578314248399
12.013377926421406,0.05807683519348606
15.351170568561873,0.04295470026773842
18.68896321070234,0.03394489531752568
22.02675585284281,0.02799571728048214
25.36454849498328,0.023787347942628878
28.702341137123746,0.020659645752736423
32.04013377926421,0.018247106037633885
35.37792642140468,0.0163315280491124
38.71571906354515,0.01477484795232296
42.05351170568562,0.013485565468564806
45.391304347826086,0.012400704279812472
48.72909698996656,0.011475536225657895
52.06688963210702,0.010677438850502784
55.40468227424749,0.009982071878072188
58.74247491638796,0.009370913494215045
62.080267558528426,0.008829624774761789
65.41806020066889,0.00834693527173796
68.75585284280936,0.007913866113225738
72.09364548494983,0.007523177284780124
75.4314381270903,0.007168967205236212
78.76923076923077,0.006846377866583159
82.10702341137124,0.00655137448678838
85.4448160535117,0.006280578627103329
88.78260869565217,0.006031140250828015
92.12040133779264,0.0058006385334219285
95.45819397993311,0.005587004170140011
98.79598662207358,0.005388457940366059
102.13377926421404,0.005203461701378065
105.47157190635451,0.005030678975440238
108.80936454849498,0.004868943013373182
112.14715719063545,0.00471723073014066
115.48494983277592,0.004574641294399396
118.82274247491638,0.004440378429818613
122.16053511705685,0.004313735701213549
125.49832775919732,0.00419408421268767
128.83612040133778,0.004080862271435936
132.17391304347825,0.0039735666595736826
135.51170568561872,0.0038717452297934254
138.8494983277592,0.0037749905973948465
142.18729096989966,0.003682934742703018
145.52508361204013,0.0035952443763747517
148.8628762541806,0.003511616942331679
152.20066889632108,0.0034317771607770015
155.53846153846155,0.003355474026159448
158.87625418060202,0.0032824781931363126
162.2140468227425,0.0032125796926808377
165.55183946488293,0.0031455859308679736
168.8896321070234,0.0030813199303415034
172.22742474916387,0.0030196187811014673
175.56521739130434,0.0029603322718957177
178.90301003344482,0.0029033216777526417
182.2408026755853,0.0028484586844278663
185.57859531772576,0.0027956244303139147
188.91638795986623,0.002744708653793271
192.2541806020067,0.002695608929247494
195.59197324414717,0.002648229984368301
198.9297658862876,0.002602483086656266
202.26755852842808,0.0025582854932603614
205.60535117056855,0.002515559953509589
208.94314381270902,0.002474234261892986
212.2809364548495,0.002434240852690665
215.61872909698997,0.0023955164339690476
218.95652173913044,0.0023580016552035804
222.2943143812709,0.0023216408055301858
225.63210702341138,0.002286381538744334
228.96989966555185,0.002252174623987525
232.30769230769232,0.002218973717495315
235.64548494983276,0.0021867351536471987
238.98327759197323,0.0021554177552435736
242.3210702341137,0.0021249826582952656
245.65886287625418,0.0020953931522063145
248.99665551839465,0.0020666145329839253
252.33444816053512,0.0020386139676711696
255.6722408026756,0.002011360370475636
259.01003344481603,0.0019848242880012804
262.3478260869565,0.0019589777935123376
265.685618729097,0.0019337943893598852
269.02341137123744,0.0019092489170734475
272.3612040133779,0.0018853174735069035
275.6989966555184,0.00186197733377688
279.03678929765886,0.0018392068798759147
282.3745819397993,0.001816985533254268
285.7123745819398,0.0017952936943382636
289.05016722408027,0.0017741126841169888
292.38795986622074,0.001753424691131406
295.7257525083612,0.0017332127218003684
299.0635451505017,0.0017134605536344094
302.40133779264215,0.0016941526926126094
305.7391304347826,0.0016752743323072163
309.0769230769231,0.0016568113163786154
312.41471571906357,0.0016387501034472603
315.75250836120404,0.0016210777337578226
319.0903010033445,0.001603781798493594
322.428093645485,0.0015868504107877665
325.7658862876254,0.0015702721786413133
329.10367892976586,0.0015540361795015846
332.44147157190633,0.001538131936141488
335.7792642140468,0.001522549394364411
339.1170568561873,0.0015072789018259968
342.45484949832775,0.0014923111881787257
345.7926421404682,0.0014776373464923333
349.1304347826087,0.0014632488152923997
352.46822742474916,0.0014491373624520131
355.80602006688963,0.0014352950691582872
359.1438127090301,0.0014217143151020208
362.4816053511706,0.0014083877651290741
365.81939799331104,0.0013953083552794595
369.1571906354515,0.0013824692809383961
372.494983277592,0.0013698639844690473
375.83277591973246,0.0013574861450390203
379.1705685618729,0.0013453296670023127
382.5083612040134,0.0013333886706863888
385.84615384615387,0.001321657482589941
389.18394648829434,0.0013101306265072906
392.5217391304348,0.0012988028150171377
395.8595317725752,0.0012876689414291762
399.1973244147157,0.001276724072160276
402.53511705685617,0.001265963439600791
405.87290969899664,0.0012553824347113934
409.2107023411371,0.0012449766010252156
412.5484949832776,0.0012347416283496485
415.88628762541805,0.0012246733462400558
419.2240802675585,0.0012147677189441304
422.561872909699,0.0012050208402285415
425.89966555183946,0.0011954289272405284
429.23745819397993,0.001185988316773426
432.5752508361204,0.001176695460047504
435.9130434782609,0.001167546917911327
439.25083612040135,0.0011585393575683325
442.5886287625418,0.0011496695478302437
445.9264214046823,0.0011409343553356408
449.26421404682276,0.0011323307410439243
452.60200668896323,0.001123855756717373
455.9397993311037,0.0011155065413642172
459.27759197324417,0.0011072803183283483
462.61538461538464,0.0010991743918038097
465.95317725752506,0.0010911861443210597
469.2909698996655,0.001083313033888495
472.628762541806,0.0010755525908212181
475.96655518394647,0.0010679024156778842
479.30434782608694,0.0010603601768477556
482.6421404682274,0.0010529236075665855
485.9799331103679,0.0010455905043615116
489.31772575250835,0.0010383587244527884
492.6555183946488,0.0010312261838010854
495.9933110367893,0.0010241908551010344
499.33110367892976,0.0010172507658597358
502.66889632107024,0.0010104039965560796
506.0066889632107,0.001003648678876963
509.3444816053512,0.00099698299402671
512.6822742474917,0.0009904051711061876
516.0200668896321,0.000983913485558309
519.3578595317725,0.0009775062576451005
522.695652173913,0.0009711818509276338
526.0334448160535,0.0009649386709681997
529.371237458194,0.000958775164114292
532.7090301003344,0.0009526898156961613
536.0468227424749,0.0009466811497678241
539.3846153846154,0.0009407477266001701
542.7224080267558,0.0009348881428708379
546.0602006688963,0.0009291010296749976
549.3979933110368,0.0009233850514312262
552.7357859531772,0.0009177389057851746
556.0735785953177,0.0009121613214340221
559.4113712374582,0.0009066510578851873
562.7491638795987,0.0009012069045318978
566.0869565217391,0.0008958276794736439
569.4247491638796,0.000890512228715046
572.7625418060201,0.0008852594256328961
576.1003344481605,0.0008800681698972806
579.438127090301,0.0008749373865899141
582.7759197324415,0.000869866025997705
586.113712374582,0.0008648530622788428
589.4515050167224,0.0008598974933254127
592.7892976588629,0.0008549983395098128
596.1270903010034,0.0008501546435971654
599.4648829431438,0.0008453654697954005
602.8026755852843,0.0008406299031420997
606.1404682274248,0.0008359470492722231
609.4782608695652,0.0008313160332963584
612.8160535117057,0.0008267359998065333
616.1538461538462,0.0008222061121178466
619.4916387959867,0.0008177255512928457
622.8294314381271,0.0008132935168140128
626.1672240802676,0.0008089092249356331
629.5050167224081,0.0008045719088046071
632.8428093645485,0.0008002808178954661
636.180602006689,0.0007960352175770406
639.5183946488295,0.0007918343885620612
642.85618729097,0.0007876776269799732
646.1939799331103,0.00078356424334551
649.5317725752508,0.0007794935625513046
652.8695652173913,0.0007754649234205427
656.2073578595317,0.0007714776783513576
659.5451505016722,0.0007675311929725438
662.8829431438127,0.0007636248458101696
666.2207357859531,0.0007597580280746321
669.5585284280936,0.0007559301428043156
672.8963210702341,0.0007521406056085533
676.2341137123746,0.0007483888430842442
679.571906354515,0.000744674293799169
682.9096989966555,0.0007409964069920352
686.247491638796,0.0007373546428355382
689.5852842809364,0.0007337484720990703
692.9230769230769,0.0007301773757457278
696.2608695652174,0.0007266408446023268
699.5986622073578,0.0007231383797909568
702.9364548494983,0.0007196694916567839
706.2742474916388,0.0007162336997338079
709.6120401337793,0.000712830533056297
712.9498327759197,0.000709459529269408
716.2876254180602,0.000706120234909952
719.6254180602007,0.0007028122046129646
722.9632107023411,0.0006995350018481949
726.3010033444816,0.0006962881977999928
729.6387959866221,0.0006930713717291752
732.9765886287626,0.0006898841105098475
736.314381270903,0.0006867260085960428
739.6521739130435,0.0006835966679888411
742.989966555184,0.0006804956976200954
746.3277591973244,0.0006774227135874574
749.6655518394649,0.0006743773389706128
753.0033444816054,0.0006713592035975795
756.3411371237459,0.0006683679438165827
759.6789297658863,0.0006654032022071553
763.0167224080268,0.0006624646281536743
766.3545150501673,0.0006595518765749088
769.6923076923077,0.0006566646089957614
773.0301003344482,0.0006538024924859159
776.3678929765887,0.0006509652000275085
779.7056856187291,0.0006481524102874338
783.0434782608696,0.0006453638070571008
786.38127090301,0.0006425990801559927
789.7190635451504,0.000639857924344035
793.0568561872909,0.000637140039499573
796.3946488294314,0.000634445130674305
799.7324414715719,0.000631772907972747
803.0702341137123,0.0006291230862829861
806.4080267558528,0.0006264953851086529
809.7458193979933,0.0006238895286980796
813.0836120401337,0.0006213052460645757
816.4214046822742,0.0006187422703807788
819.7591973244147,0.0006162003394416042
823.0969899665552,0.0006136791952604619
826.4347826086956,0.0006111785837154679
829.7725752508361,0.0006086982554632588
833.1103678929766,0.0006062379646251984
836.448160535117,0.0006037974694583303
839.7859531772575,0.0006013765322074282
843.123745819398,0.0005989749187976885
846.4615384615385,0.0005965923987989499
849.7993311036789,0.0005942287456220132
853.1371237458194,0.0005918837359998653
856.4749163879599,0.0005895571504572313
859.8127090301003,0.0005872487726644979
863.1505016722408,0.0005849583899323443
866.4882943143813,0.0005826857927624164
869.8260869565217,0.0005804307747104396
873.1638795986622,0.0005781931327147017
876.5016722408027,0.0005759726670094315
879.8394648829432,0.0005737691804470358
883.1772575250836,0.0005715824790401095
886.5150501672241,0.0005694123719880021
889.8528428093646,0.0005672586711668283
893.190635451505,0.0005651211911571637
896.5284280936455,0.0005629997496122644
899.866220735786,0.0005608941666548579
903.2040133779265,0.0005588042653883318
906.5418060200669,0.0005567298710070164
909.8795986622074,0.0005546708119825082
913.2173913043479,0.0005526269187263985
916.5551839464883,0.0005505980243832745
919.8929765886288,0.0005485839646857951
923.2307692307693,0.00054658457742372
926.5685618729098,0.0005445997028924558
929.9063545150501,0.0005426291839209008
933.2441471571906,0.0005406728651826104
936.581939799331,0.0005387305937552849
939.9197324414715,0.0005368022191106341
943.257525083612,0.0005348875926331296
946.5953177257525,0.0005329865678949013
949.9331103678929,0.00053109900042849
953.2709030100334,0.0005292247479874111
956.6086956521739,0.0005273636702455618
959.9464882943143,0.0005255156286943427
963.2842809364548,0.0005236804870229984
966.6220735785953,0.0005218581106862949
969.9598662207358,0.0005200483668619547
973.2976588628762,0.0005182511248392943
976.6354515050167,0.0005164662555531645
979.9732441471572,0.0005146936316337394
983.3110367892976,0.0005129331277323195
986.6488294314381,0.0005111846196876483
989.9866220735786,0.0005094479856679211
993.3244147157191,0.0005077231050071281
996.6622073578595,0.0005060098588972451
1000.0,0.0005043081300583359

==> sections/0_Abstract.tex <==
\abstract{The Bregman distance is a central tool in convex optimization, particularly in first-order gradient descent and proximal-based algorithms. Such methods enable optimization of functions without Lipschitz continuous gradients by leveraging the concept of relative smoothness, with respect to a reference function $h$. A key factor in determining the full range of allowed step sizes in Bregman schemes is the symmetry coefficient, $\alpha(h)$, of the reference function $h$. While some explicit values of $\alpha(h)$ have been determined for specific functions $h$, a general characterization has remained elusive. This paper explores two problems: (\textit{i}) deriving calculus rules for the symmetry coefficient and (\textit{ii}) computing $\alpha(\norm{\cdot}_2^p)$ for general $p$. We establish upper and lower bounds for the symmetry coefficient of sums of positively homogeneous Legendre functions and, under certain conditions, provide exact formulas for these sums. Furthermore, we demonstrate that $\alpha(\norm{\cdot}_2^p)$ is independent of dimension and propose an efficient algorithm for its computation. Additionally, we prove that $\alpha(\norm{\cdot}_2^p)$ asymptotically equals, and is lower bounded by, the function $1/(2p)$, offering a simpler upper bound for step sizes in Bregman schemes. Finally, we present closed-form computations for specific cases such as $p \in \{6,8,10\}$}
